Detection of Elements at All Three r-process Peaks in the Metal-Poor Star HD 160617

We report the first detection of elements at all three r-process peaks in the metal-poor halo star HD 160617. These elements include arsenic and selenium, which have not been detected previously in halo stars, and the elements tellurium, osmium, iridium, and platinum, which have been detected previously. Absorption lines of these elements are found in archive observations made with the Space Telescope Imaging Spectrograph onboard the Hubble Space Telescope. We present up-to-date absolute atomic transition probabilities and complete line component patterns for these elements. Additional archival spectra of this star from several ground-based instruments allow us to derive abundances or upper limits of 45 elements in HD 160617, including 27 elements produced by neutron-capture reactions. The average abundances of the elements at the three r-process peaks are similar to the predicted solar system r-process residuals when scaled to the abundances in the rare earth element domain. This result for arsenic and selenium may be surprising in light of predictions that the production of the lightest r-process elements generally should be decoupled from the heavier r-process elements.

==> tab10.tex <==
Title: Detection of Elements at All Three r-process Peaks in the Metal-Poor Star
 HD 160617
Authors: Roederer I.U. and Lawler J.E.,
Table: Hyperfine structure and isotopic line component patterns for Yb II lines
================================================================================
Byte-by-byte Description of file:
--------------------------------------------------------------------------------
   Bytes Format Units Label   Explanations
--------------------------------------------------------------------------------
  1- 8   F8.2   cm-1  WaveNum Center-of-Gravity Wavenumber
  10- 17 F8.3   0.1nm WaveAir Center-of-Gravity Air Wavelength in Angstroms
  19- 21 F3.1   ---   Fupp    Component upper level F or total angular momentum
  23- 25 F3.1   ---   Flow    Component lower level F or total angular momentum
  27- 34 F8.5   cm-1  CWaveR  Component offset Wavenumber with respect to
                               Center-of-gravity Wavenumber
  36- 44 F9.6   0.1nm CWaveR  Component offset Wavelength with respect to
                               Center-of-gravity Wavelength
  46- 52 F7.5   ---   Str     Component strength (1)
  54- 56 I3     ---   Iso     Isotope
--------------------------------------------------------------------------------
Note (1): Normalized to sum to one.
--------------------------------------------------------------------------------
47005.46 2126.741 1.5 0.5 -0.07332  0.003318 0.00130 168
47005.46 2126.741 1.5 0.5 -0.04850  0.002195 0.03040 170
47005.46 2126.741 1.5 0.5 -0.01332  0.000603 0.21830 172
47005.46 2126.741 1.5 0.5  0.01432 -0.000648 0.31830 174
47005.46 2126.741 1.5 0.5  0.04068 -0.001841 0.12760 176
47005.46 2126.741 2.0 1.0 -0.14134  0.006396 0.08925 171
47005.46 2126.741 1.0 1.0 -0.14134  0.006396 0.01785 171
47005.46 2126.741 1.0 0.0  0.28037 -0.012687 0.03570 171
47005.46 2126.741 4.0 3.0  0.14495 -0.006559 0.06049 173
47005.46 2126.741 3.0 3.0  0.14495 -0.006559 0.02614 173
47005.46 2126.741 3.0 2.0 -0.20501  0.009277 0.02091 173
47005.46 2126.741 2.0 3.0  0.14495 -0.006559 0.00747 173
47005.46 2126.741 2.0 2.0 -0.20501  0.009277 0.02614 173
47005.46 2126.741 1.0 2.0 -0.20501  0.009277 0.02016 173
47228.96 2116.675 0.5 0.5 -0.07332  0.003287 0.00130 168
47228.96 2116.675 0.5 0.5 -0.04850  0.002174 0.03040 170
47228.96 2116.675 0.5 0.5 -0.01332  0.000597 0.21830 172
47228.96 2116.675 0.5 0.5  0.01432 -0.000642 0.31830 174
47228.96 2116.675 0.5 0.5  0.04068 -0.001823 0.12760 176
47228.96 2116.675 1.0 1.0 -0.14134  0.006335 0.07140 171
47228.96 2116.675 1.0 0.0  0.28037 -0.012567 0.03570 171
47228.96 2116.675 0.0 1.0 -0.14134  0.006335 0.03570 171
47228.96 2116.675 3.0 3.0  0.14495 -0.006497 0.04182 173
47228.96 2116.675 3.0 2.0 -0.20501  0.009189 0.05227 173
47228.96 2116.675 2.0 3.0  0.14495 -0.006497 0.05227 173
47228.96 2116.675 2.0 2.0 -0.20501  0.009189 0.01494 173


==> tab12.tex <==
Title: Detection of Elements at All Three r-process Peaks in the Metal-Poor Star
 HD 160617
Authors: Roederer I. U. and Lawler J.E., 
Table: Hyperfine structure and isotopic line component pattern of the 1942 
Angstrom line of Hg II.
================================================================================
Byte-by-byte Description of file: 
--------------------------------------------------------------------------------
   Bytes Format Units Label   Explanations
--------------------------------------------------------------------------------
  1-  9  F9.3   cm-1  WaveNum Center-of-Gravity Wavenumber
  11- 19 F9.4   0.1nm WaveAir Center-of-Gravity Air Wavelength in Angstroms
  21- 23 F3.1   ---   Fupp    Component upper level F or total angular momentum
  25- 27 F3.1   ---   Flow    Component lower level F or total angular momentum
  29- 36 F8.5   cm-1  CWaveR  Component offset Wavenumber with respect to
                               Center-of-gravity Wavenumber
  38- 46 F9.6   0.1nm CWaveR  Component offset Wavelength with respect to
                               Center-of-gravity Wavelength
  48- 54 F7.5   ---   Str     Component strength (1)
  56- 58 I3     ---   Iso     Isotope 
--------------------------------------------------------------------------------
Note (1): Normalized to sum to one.
--------------------------------------------------------------------------------

51486.070 1942.2729 0.5 0.5  0.44405 -0.016751 0.00150 196
51486.070 1942.2729 0.5 0.5  0.24705 -0.009320 0.09970 198
51486.070 1942.2729 0.5 0.5  0.05005 -0.001888 0.23100 200
51486.070 1942.2729 0.5 0.5 -0.16095  0.006072 0.29860 202
51486.070 1942.2729 0.5 0.5 -0.36795  0.013881 0.06870 204
51486.070 1942.2729 1.0 1.0 -0.05424  0.002046 0.08435 199
51486.070 1942.2729 1.0 0.0  1.29694 -0.048925 0.04217 199
51486.070 1942.2729 0.0 1.0 -0.28624  0.010798 0.04217 199
51486.070 1942.2729 2.0 2.0  0.29749 -0.011223 0.04119 201
51486.070 1942.2729 2.0 1.0 -0.70168  0.026471 0.04119 201
51486.070 1942.2729 1.0 2.0  0.47149 -0.017787 0.04119 201
51486.070 1942.2729 1.0 1.0 -0.52768  0.019906 0.00824 201


==> tab13.tex <==
\begin{deluxetable}{cccccc}
\tablecaption{Equivalent width measurements
\label{ewtab}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
%\rotate
\tablehead{
\colhead{Wavelength (\AA)} &
\colhead{Species} &
\colhead{E.P. (eV)} &
\colhead{log($gf$)} &
\colhead{EW (m\AA)} &
\colhead{Instrument} }
\startdata
   5682.63                  & Na~\textsc{i} &   2.100  &  -0.706   &    5.3 & HARPS \\
   5688.20                  & Na~\textsc{i} &   2.100  &  -0.452   &   14.3 & HARPS \\
   4167.27                  & Mg~\textsc{i} &   4.346  &  -0.710   &   58.1 & HARPS \\
   4702.99                  & Mg~\textsc{i} &   4.330  &  -0.380   &   79.3 & HARPS \\
   5528.40                  & Mg~\textsc{i} &   4.340  &  -0.498   &   73.7 & HARPS \\
   5711.09                  & Mg~\textsc{i} &   4.340  &  -1.724   &   11.4 & HARPS \\
   5701.10                  & Si~\textsc{i} &   4.930  &  -1.740   &    1.7 & HARPS \\
   5708.40                  & Si~\textsc{i} &   4.930  &  -1.470   &    5.9 & HARPS \\
   5772.15                  & Si~\textsc{i} &   5.060  &  -1.740   &    2.1 & HARPS \\
   4283.01                  & Ca~\textsc{i} &   1.886  &  -0.224   &   62.3 & HARPS \\
   4318.65                  & Ca~\textsc{i} &   1.890  &  -0.210   &   57.0 & HARPS \\
   4425.44                  & Ca~\textsc{i} &   1.879  &  -0.358   &   51.3 & HARPS \\
   4434.96                  & Ca~\textsc{i} &   1.886  &  -0.010   &   67.0 & HARPS \\
   4435.69                  & Ca~\textsc{i} &   1.890  &  -0.519   &   45.9 & HIRES \\
   4454.78                  & Ca~\textsc{i} &   1.898  &   0.260   &   79.4 & HARPS \\
   4455.89                  & Ca~\textsc{i} &   1.899  &  -0.530   &   45.1 & HARPS \\
   5588.76                  & Ca~\textsc{i} &   2.520  &   0.210   &   58.5 & HARPS \\
   5857.45                  & Ca~\textsc{i} &   2.930  &   0.230   &   35.3 & HARPS \\
   6102.72                  & Ca~\textsc{i} &   1.880  &  -0.850   &   32.0 & HARPS \\
   6122.22                  & Ca~\textsc{i} &   1.890  &  -0.380   &   63.2 & HARPS \\
   6162.17                  & Ca~\textsc{i} &   1.900  &  -0.170   &   76.2 & HARPS \\
   6439.07                  & Ca~\textsc{i} &   2.520  &   0.470   &   60.5 & HARPS \\
   3998.64                  & Ti~\textsc{i} &   0.048  &   0.010   &   45.3 & HARPS \\
   4512.73                  & Ti~\textsc{i} &   0.840  &  -0.424   &    7.1 & HARPS \\
   4518.02                  & Ti~\textsc{i} &   0.830  &  -0.269   &    8.9 & HARPS \\
   4533.25                  & Ti~\textsc{i} &   0.848  &   0.532   &   37.1 & HARPS \\
   4534.78                  & Ti~\textsc{i} &   0.840  &   0.336   &   26.6 & HARPS \\
   4548.76                  & Ti~\textsc{i} &   0.830  &  -0.298   &    8.4 & HARPS \\
   4555.49                  & Ti~\textsc{i} &   0.850  &  -0.432   &    5.6 & HARPS \\
   4656.47                  & Ti~\textsc{i} &   0.000  &  -1.289   &    6.7 & HARPS \\
   4681.91                  & Ti~\textsc{i} &   0.048  &  -1.015   &    8.5 & HARPS \\
   4840.87                  & Ti~\textsc{i} &   0.900  &  -0.453   &    6.8 & HARPS \\
   4981.73                  & Ti~\textsc{i} &   0.840  &   0.560   &   38.8 & HARPS \\
   4999.50                  & Ti~\textsc{i} &   0.830  &   0.306   &   28.7 & HARPS \\
   5016.16                  & Ti~\textsc{i} &   0.850  &  -0.518   &    5.4 & HARPS \\
   5064.65\tablenotemark{a} & Ti~\textsc{i} &   0.050  &  -0.935   &   14.9 & HARPS \\
   5173.74                  & Ti~\textsc{i} &   0.000  &  -1.062   &   10.8 & HARPS \\
   5192.97                  & Ti~\textsc{i} &   0.020  &  -0.950   &   12.9 & HARPS \\
   5210.39                  & Ti~\textsc{i} &   0.050  &  -0.828   &   15.0 & HARPS \\
   3321.70                  & Ti~\textsc{ii}&   1.230  &  -0.310   &   71.4 & UVES  \\
   3343.76                  & Ti~\textsc{ii}&   0.150  &  -1.150   &   83.8 & UVES  \\
   3456.38\tablenotemark{a} & Ti~\textsc{ii}&   2.060  &  -0.100   &   46.6 & UVES  \\
   3491.05                  & Ti~\textsc{ii}&   0.110  &  -1.150   &   89.8 & UVES  \\
   4028.34                  & Ti~\textsc{ii}&   1.890  &  -0.960   &   37.9 & HARPS \\
   4337.91\tablenotemark{a} & Ti~\textsc{ii}&   1.080  &  -0.960   &   64.7 & HARPS \\
   4394.06                  & Ti~\textsc{ii}&   1.221  &  -1.780   &   29.9 & HARPS \\
   4395.03                  & Ti~\textsc{ii}&   1.080  &  -0.540   &   89.3 & HARPS \\
   4395.84                  & Ti~\textsc{ii}&   1.243  &  -1.930   &   20.4 & HARPS \\
   4398.29\tablenotemark{a} & Ti~\textsc{ii}&   1.210  &  -2.650   &    2.6 & HARPS \\
   4399.77                  & Ti~\textsc{ii}&   1.240  &  -1.190   &   58.6 & HARPS \\
   4409.52\tablenotemark{a} & Ti~\textsc{ii}&   1.230  &  -2.370   &    5.6 & HARPS \\
   4417.71                  & Ti~\textsc{ii}&   1.165  &  -1.190   &   62.1 & HARPS \\
   4418.33                  & Ti~\textsc{ii}&   1.240  &  -1.970   &   21.8 & HARPS \\
   4443.80                  & Ti~\textsc{ii}&   1.080  &  -0.720   &   87.5 & HARPS \\
   4444.55                  & Ti~\textsc{ii}&   1.120  &  -2.240   &   16.6 & HARPS \\
   4450.48                  & Ti~\textsc{ii}&   1.080  &  -1.520   &   50.9 & HARPS \\
   4464.45                  & Ti~\textsc{ii}&   1.160  &  -1.810   &   32.3 & HARPS \\
   4470.85                  & Ti~\textsc{ii}&   1.165  &  -2.020   &   18.4 & HARPS \\
   4493.52\tablenotemark{a} & Ti~\textsc{ii}&   1.080  &  -3.020   &    6.1 & HARPS \\
   4501.27\tablenotemark{a} & Ti~\textsc{ii}&   1.116  &  -0.770   &   86.2 & HARPS \\
   4533.96                  & Ti~\textsc{ii}&   1.240  &  -0.530   &   87.0 & HARPS \\
   4571.97                  & Ti~\textsc{ii}&   1.572  &  -0.320   &   83.2 & HARPS \\
   4583.41                  & Ti~\textsc{ii}&   1.160  &  -2.920   &    3.5 & HARPS \\
   4636.32                  & Ti~\textsc{ii}&   1.160  &  -3.020   &    2.5 & HARPS \\
   4657.20                  & Ti~\textsc{ii}&   1.240  &  -2.240   &   12.5 & HARPS \\
   4708.66                  & Ti~\textsc{ii}&   1.240  &  -2.340   &   12.2 & HARPS \\
   4798.53                  & Ti~\textsc{ii}&   1.080  &  -2.680   &    9.2 & HARPS \\
   5129.16                  & Ti~\textsc{ii}&   1.890  &  -1.240   &   22.4 & HARPS \\
   5185.90                  & Ti~\textsc{ii}&   1.890  &  -1.490   &   19.5 & HARPS \\
   5226.54                  & Ti~\textsc{ii}&   1.570  &  -1.260   &   41.4 & HARPS \\
   5336.79                  & Ti~\textsc{ii}&   1.580  &  -1.590   &   24.1 & HARPS \\
   5381.02                  & Ti~\textsc{ii}&   1.570  &  -1.920   &   13.7 & HARPS \\
   5418.77                  & Ti~\textsc{ii}&   1.580  &  -2.000   &    9.5 & HARPS \\
   3578.68                  & Cr~\textsc{i} &   0.000  &   0.420   &   93.7 & UVES  \\
   4274.80                  & Cr~\textsc{i} &   0.000  &  -0.220   &   87.6 & HARPS \\
   4289.72                  & Cr~\textsc{i} &   0.000  &  -0.370   &   75.2 & HARPS \\
   4545.95                  & Cr~\textsc{i} &   0.940  &  -1.370   &    9.6 & HARPS \\
   4646.15                  & Cr~\textsc{i} &   1.030  &  -0.740   &   24.3 & HARPS \\
   4651.28                  & Cr~\textsc{i} &   0.980  &  -1.460   &    5.8 & HARPS \\
   4789.34                  & Cr~\textsc{i} &   2.540  &  -0.330   &    3.3 & HARPS \\
   5206.04                  & Cr~\textsc{i} &   0.940  &   0.020   &   61.6 & HARPS \\
   5296.69                  & Cr~\textsc{i} &   0.980  &  -1.360   &    8.0 & HARPS \\
   5298.28                  & Cr~\textsc{i} &   0.980  &  -1.140   &   11.4 & HARPS \\
   5345.80                  & Cr~\textsc{i} &   1.000  &  -0.950   &   17.5 & HARPS \\
   5348.31                  & Cr~\textsc{i} &   1.000  &  -1.210   &    9.7 & HARPS \\
   5409.77                  & Cr~\textsc{i} &   1.030  &  -0.670   &   26.8 & HARPS \\
   4558.59                  & Cr~\textsc{ii}&   4.070  &  -0.656   &   27.4 & HARPS \\
   4588.14                  & Cr~\textsc{ii}&   4.070  &  -0.826   &   18.0 & HARPS \\
   4591.99                  & Cr~\textsc{ii}&   4.070  &  -1.419   &    6.4 & HARPS \\
   3786.68\tablenotemark{a} & Fe~\textsc{i} &   1.010  &  -2.185   &   48.8 & HARPS \\
   3787.88\tablenotemark{a} & Fe~\textsc{i} &   1.010  &  -0.838   &   97.2 & HARPS \\
   3805.34\tablenotemark{a} & Fe~\textsc{i} &   3.300  &   0.313   &   59.9 & HARPS \\
   3815.84\tablenotemark{a} & Fe~\textsc{i} &   1.480  &   0.237   &  147.6 & HARPS \\
   3840.44\tablenotemark{a} & Fe~\textsc{i} &   0.990  &  -0.497   &  117.6 & HARPS \\
   3841.05\tablenotemark{a} & Fe~\textsc{i} &   1.610  &  -0.044   &  108.2 & HARPS \\
   3849.97                  & Fe~\textsc{i} &   1.010  &  -0.863   &  105.9 & HARPS \\
   3856.37\tablenotemark{a} & Fe~\textsc{i} &   0.052  &  -1.280   &  121.9 & HARPS \\
   3865.52                  & Fe~\textsc{i} &   1.011  &  -0.950   &  104.9 & HARPS \\
   3899.71\tablenotemark{a} & Fe~\textsc{i} &   0.090  &  -1.515   &  110.7 & HARPS \\
   3902.95\tablenotemark{a} & Fe~\textsc{i} &   1.560  &  -0.442   &  100.5 & HARPS \\
   3920.26                  & Fe~\textsc{i} &   0.120  &  -1.734   &  103.1 & HARPS \\
   3922.91                  & Fe~\textsc{i} &   0.050  &  -1.626   &  111.8 & HARPS \\
   3949.95                  & Fe~\textsc{i} &   2.180  &  -1.251   &   49.2 & HARPS \\
   4005.24\tablenotemark{a} & Fe~\textsc{i} &   1.557  &  -0.583   &   92.9 & HARPS \\
   4114.44                  & Fe~\textsc{i} &   2.831  &  -1.303   &   20.5 & HARPS \\
   4134.68                  & Fe~\textsc{i} &   2.830  &  -0.649   &   50.2 & HARPS \\
   4143.87                  & Fe~\textsc{i} &   1.557  &  -0.511   &  102.6 & HARPS \\
   4147.67                  & Fe~\textsc{i} &   1.480  &  -2.071   &   42.9 & HARPS \\
   4154.50                  & Fe~\textsc{i} &   2.830  &  -0.688   &   43.6 & HARPS \\
   4157.78                  & Fe~\textsc{i} &   3.420  &  -0.403   &   32.3 & HARPS \\
   4174.91                  & Fe~\textsc{i} &   0.910  &  -2.938   &   30.1 & HARPS \\
   4175.64                  & Fe~\textsc{i} &   2.845  &  -0.827   &   42.7 & HARPS \\
   4181.76                  & Fe~\textsc{i} &   2.830  &  -0.371   &   61.6 & HARPS \\
   4182.38                  & Fe~\textsc{i} &   3.020  &  -1.180   &   16.9 & HARPS \\
   4184.89                  & Fe~\textsc{i} &   2.830  &  -0.869   &   38.7 & HARPS \\
   4187.04                  & Fe~\textsc{i} &   2.449  &  -0.514   &   70.5 & HARPS \\
   4191.43                  & Fe~\textsc{i} &   2.470  &  -0.666   &   63.5 & HARPS \\
   4195.33                  & Fe~\textsc{i} &   3.330  &  -0.492   &   33.0 & HARPS \\
   4199.10                  & Fe~\textsc{i} &   3.047  &   0.156   &   69.4 & HARPS \\
   4202.03                  & Fe~\textsc{i} &   1.485  &  -0.689   &   95.6 & HARPS \\
   4216.18                  & Fe~\textsc{i} &   0.000  &  -3.357   &   53.5 & HARPS \\
   4217.55                  & Fe~\textsc{i} &   3.430  &  -0.484   &   29.1 & HARPS \\
   4222.21                  & Fe~\textsc{i} &   2.449  &  -0.914   &   52.5 & HARPS \\
   4233.60                  & Fe~\textsc{i} &   2.482  &  -0.579   &   66.3 & HARPS \\
   4238.81                  & Fe~\textsc{i} &   3.400  &  -0.233   &   40.9 & HARPS \\
   4250.12                  & Fe~\textsc{i} &   2.469  &  -0.380   &   77.2 & HARPS \\
   4250.79                  & Fe~\textsc{i} &   1.557  &  -0.713   &   96.7 & HARPS \\
   4260.47\tablenotemark{a} & Fe~\textsc{i} &   2.400  &   0.077   &   98.5 & HARPS \\
   4271.15                  & Fe~\textsc{i} &   2.449  &  -0.337   &   80.1 & HARPS \\
   4271.76\tablenotemark{a} & Fe~\textsc{i} &   1.485  &  -0.173   &  125.0 & HARPS \\
   4282.40                  & Fe~\textsc{i} &   2.176  &  -0.779   &   66.2 & HARPS \\
   4375.93\tablenotemark{a} & Fe~\textsc{i} &   0.000  &  -3.005   &   69.8 & HARPS \\
   4388.41                  & Fe~\textsc{i} &   3.600  &  -0.681   &   18.2 & HARPS \\
   4404.75\tablenotemark{a} & Fe~\textsc{i} &   1.557  &  -0.147   &  124.3 & HARPS \\
   4415.12                  & Fe~\textsc{i} &   1.608  &  -0.621   &  102.9 & HARPS \\
   4427.31\tablenotemark{a} & Fe~\textsc{i} &   0.050  &  -2.924   &   71.2 & HARPS \\
   4461.65\tablenotemark{a} & Fe~\textsc{i} &   0.090  &  -3.194   &   58.7 & HARPS \\
   4442.34                  & Fe~\textsc{i} &   2.198  &  -1.228   &   54.2 & HARPS \\
   4443.19                  & Fe~\textsc{i} &   2.858  &  -1.043   &   29.7 & HARPS \\
   4447.72                  & Fe~\textsc{i} &   2.223  &  -1.339   &   46.1 & HARPS \\
   4466.55                  & Fe~\textsc{i} &   2.830  &  -0.600   &   51.1 & HARPS \\
   4489.74                  & Fe~\textsc{i} &   0.121  &  -3.899   &   20.9 & HARPS \\
   4494.56                  & Fe~\textsc{i} &   2.198  &  -1.143   &   57.2 & HARPS \\
   4531.15                  & Fe~\textsc{i} &   1.480  &  -2.101   &   41.8 & HARPS \\
   4592.65                  & Fe~\textsc{i} &   1.560  &  -2.462   &   27.9 & HIRES \\
   4595.36                  & Fe~\textsc{i} &   3.290  &  -1.758   &    3.6 & HIRES \\
   4602.94                  & Fe~\textsc{i} &   1.485  &  -2.208   &   41.2 & HARPS \\
   4630.12                  & Fe~\textsc{i} &   2.280  &  -2.587   &    5.8 & HARPS \\
   4643.46                  & Fe~\textsc{i} &   3.640  &  -1.147   &    5.9 & HARPS \\
   4647.43                  & Fe~\textsc{i} &   2.950  &  -1.351   &   18.3 & HARPS \\
   4733.59                  & Fe~\textsc{i} &   1.490  &  -2.988   &   11.4 & HARPS \\
   4736.77                  & Fe~\textsc{i} &   3.211  &  -0.752   &   32.8 & HARPS \\
   4786.81                  & Fe~\textsc{i} &   3.000  &  -1.606   &    9.2 & HARPS \\
   4789.65                  & Fe~\textsc{i} &   3.530  &  -0.957   &   13.7 & HARPS \\
   4800.65                  & Fe~\textsc{i} &   4.120  &  -1.028   &    2.6 & HARPS \\
   4871.32                  & Fe~\textsc{i} &   2.870  &  -0.362   &   60.5 & HARPS \\
   4872.14                  & Fe~\textsc{i} &   2.882  &  -0.567   &   50.6 & HARPS \\
   4890.76                  & Fe~\textsc{i} &   2.876  &  -0.394   &   60.0 & HARPS \\
   4891.49                  & Fe~\textsc{i} &   2.852  &  -0.111   &   73.9 & HARPS \\
   4903.31                  & Fe~\textsc{i} &   2.880  &  -0.926   &   36.8 & HARPS \\
   4918.99                  & Fe~\textsc{i} &   2.845  &  -0.342   &   65.5 & HARPS \\
   4920.50                  & Fe~\textsc{i} &   2.832  &   0.068   &   86.2 & HARPS \\
   4924.77                  & Fe~\textsc{i} &   2.280  &  -2.114   &   11.7 & HARPS \\
   4938.81                  & Fe~\textsc{i} &   2.875  &  -1.077   &   28.5 & HARPS \\
   4939.69                  & Fe~\textsc{i} &   0.859  &  -3.252   &   18.6 & HARPS \\
   4966.09                  & Fe~\textsc{i} &   3.330  &  -0.871   &   23.6 & HARPS \\
   4994.13                  & Fe~\textsc{i} &   0.920  &  -2.969   &   29.2 & HARPS \\
   5006.12                  & Fe~\textsc{i} &   2.830  &  -0.615   &   51.8 & HARPS \\
   5028.13                  & Fe~\textsc{i} &   3.560  &  -1.122   &    7.6 & HARPS \\
   5044.21                  & Fe~\textsc{i} &   2.850  &  -2.017   &    4.3 & HARPS \\
   5049.82                  & Fe~\textsc{i} &   2.280  &  -1.355   &   43.1 & HARPS \\
   5051.63                  & Fe~\textsc{i} &   0.920  &  -2.764   &   41.0 & HARPS \\
   5068.77                  & Fe~\textsc{i} &   2.940  &  -1.041   &   29.1 & HARPS \\
   5079.22                  & Fe~\textsc{i} &   2.200  &  -2.105   &   19.2 & HARPS \\
   5079.74\tablenotemark{a} & Fe~\textsc{i} &   0.990  &  -3.245   &   20.6 & HARPS \\
   5083.34                  & Fe~\textsc{i} &   0.960  &  -2.842   &   32.1 & HARPS \\
   5123.72                  & Fe~\textsc{i} &   1.010  &  -3.058   &   24.5 & HARPS \\
   5127.36                  & Fe~\textsc{i} &   0.920  &  -3.249   &   19.7 & HARPS \\
   5131.47                  & Fe~\textsc{i} &   2.220  &  -2.515   &    6.6 & HARPS \\
   5141.74                  & Fe~\textsc{i} &   2.420  &  -2.238   &    8.8 & HARPS \\
   5150.84                  & Fe~\textsc{i} &   0.990  &  -3.037   &   22.8 & HARPS \\
   5151.91                  & Fe~\textsc{i} &   1.010  &  -3.321   &   16.2 & HARPS \\
   5166.28                  & Fe~\textsc{i} &   0.000  &  -4.123   &   21.0 & HARPS \\
   5171.60                  & Fe~\textsc{i} &   1.490  &  -1.721   &   61.9 & HARPS \\
   5191.45                  & Fe~\textsc{i} &   3.040  &  -0.551   &   44.7 & HIRES \\
   5192.34                  & Fe~\textsc{i} &   3.000  &  -0.421   &   54.0 & HARPS \\
   5194.94                  & Fe~\textsc{i} &   1.560  &  -2.021   &   45.7 & HARPS \\
   5198.71                  & Fe~\textsc{i} &   2.220  &  -2.091   &   15.5 & HARPS \\
   5202.34\tablenotemark{a} & Fe~\textsc{i} &   2.180  &  -1.871   &   30.0 & HARPS \\
   5216.27                  & Fe~\textsc{i} &   1.610  &  -2.082   &   39.2 & HARPS \\
   5217.39                  & Fe~\textsc{i} &   3.210  &  -1.162   &   16.8 & HARPS \\
   5225.53                  & Fe~\textsc{i} &   0.110  &  -4.755   &    4.3 & HARPS \\
   5232.94                  & Fe~\textsc{i} &   2.940  &  -0.057   &   73.3 & HARPS \\
   5242.49                  & Fe~\textsc{i} &   3.630  &  -0.967   &   10.8 & HARPS \\
   5266.56                  & Fe~\textsc{i} &   3.000  &  -0.385   &   56.4 & HARPS \\
   5269.54\tablenotemark{a} & Fe~\textsc{i} &   0.860  &  -1.333   &  109.4 & HARPS \\
   5281.79                  & Fe~\textsc{i} &   3.040  &  -0.833   &   32.7 & HARPS \\
   5283.62                  & Fe~\textsc{i} &   3.240  &  -0.524   &   41.2 & HARPS \\
   5288.53\tablenotemark{a} & Fe~\textsc{i} &   3.680  &  -1.508   &    2.1 & HARPS \\
   5307.36                  & Fe~\textsc{i} &   1.610  &  -2.912   &    8.3 & HIRES \\
   5332.90\tablenotemark{a} & Fe~\textsc{i} &   1.550  &  -2.776   &   11.6 & HIRES \\
   5339.93                  & Fe~\textsc{i} &   3.270  &  -0.720   &   31.3 & HARPS \\
   5364.87                  & Fe~\textsc{i} &   4.450  &   0.228   &   23.6 & HARPS \\
   5365.40\tablenotemark{a} & Fe~\textsc{i} &   3.560  &  -1.020   &    6.7 & HARPS \\
   5367.47                  & Fe~\textsc{i} &   4.420  &   0.443   &   29.2 & HARPS \\
   5369.96\tablenotemark{a} & Fe~\textsc{i} &   4.370  &   0.536   &   32.6 & HARPS \\
   5371.49\tablenotemark{a} & Fe~\textsc{i} &   0.960  &  -1.644   &   95.2 & HARPS \\
   5379.57                  & Fe~\textsc{i} &   3.690  &  -1.514   &    2.5 & HARPS \\
   5383.37\tablenotemark{a} & Fe~\textsc{i} &   4.310  &   0.645   &   39.7 & HARPS \\
   5397.13\tablenotemark{a} & Fe~\textsc{i} &   0.920  &  -1.982   &   82.4 & HARPS \\
   5405.77\tablenotemark{a} & Fe~\textsc{i} &   0.990  &  -1.852   &   83.9 & HARPS \\
   5410.91                  & Fe~\textsc{i} &   4.470  &   0.398   &   25.1 & HARPS \\
   5415.20\tablenotemark{a} & Fe~\textsc{i} &   4.390  &   0.643   &   37.0 & HARPS \\
   5429.70\tablenotemark{a} & Fe~\textsc{i} &   0.960  &  -1.881   &   89.5 & HIRES \\
   5497.52                  & Fe~\textsc{i} &   1.010  &  -2.825   &   36.2 & HARPS \\
   5501.47                  & Fe~\textsc{i} &   0.960  &  -3.046   &   28.8 & HARPS \\
   5506.78                  & Fe~\textsc{i} &   0.990  &  -2.789   &   40.0 & HARPS \\
   5586.76                  & Fe~\textsc{i} &   3.370  &  -0.144   &   53.0 & HARPS \\
   5662.52                  & Fe~\textsc{i} &   4.180  &  -0.573   &    9.5 & HARPS \\
   5701.54                  & Fe~\textsc{i} &   2.560  &  -2.143   &    7.2 & HARPS \\
   5753.12                  & Fe~\textsc{i} &   4.260  &  -0.688   &    6.6 & HARPS \\
   5816.37\tablenotemark{a} & Fe~\textsc{i} &   4.550  &  -0.601   &    2.8 & HARPS \\
   6065.48                  & Fe~\textsc{i} &   2.610  &  -1.410   &   26.2 & HARPS \\
   6136.61                  & Fe~\textsc{i} &   2.450  &  -1.410   &   36.8 & HARPS \\
   6137.69                  & Fe~\textsc{i} &   2.590  &  -1.346   &   29.9 & HARPS \\
   6191.56                  & Fe~\textsc{i} &   2.430  &  -1.416   &   34.6 & HARPS \\
   6213.43\tablenotemark{a} & Fe~\textsc{i} &   2.220  &  -2.481   &    6.1 & HARPS \\
   6219.28                  & Fe~\textsc{i} &   2.200  &  -2.448   &   10.6 & HARPS \\
   6230.72\tablenotemark{a} & Fe~\textsc{i} &   2.560  &  -1.276   &   42.5 & HARPS \\
   6246.32                  & Fe~\textsc{i} &   3.600  &  -0.877   &   17.1 & HARPS \\
   6265.13                  & Fe~\textsc{i} &   2.180  &  -2.540   &    7.4 & HARPS \\
   6297.79                  & Fe~\textsc{i} &   2.220  &  -2.640   &    5.1 & HIRES \\
   6355.03\tablenotemark{a} & Fe~\textsc{i} &   2.840  &  -2.291   &    2.1 & HARPS \\
   6393.60                  & Fe~\textsc{i} &   2.430  &  -1.576   &   31.1 & HARPS \\
   6421.35                  & Fe~\textsc{i} &   2.280  &  -2.014   &   18.6 & HARPS \\
   6430.85                  & Fe~\textsc{i} &   2.180  &  -1.946   &   22.7 & HARPS \\
   6494.98                  & Fe~\textsc{i} &   2.400  &  -1.239   &   48.4 & HARPS \\
   6592.91                  & Fe~\textsc{i} &   2.730  &  -1.473   &   19.9 & HIRES \\
   6593.87                  & Fe~\textsc{i} &   2.440  &  -2.366   &    6.0 & HARPS \\
   6677.99                  & Fe~\textsc{i} &   2.690  &  -1.418   &   29.2 & HARPS \\
   6750.15                  & Fe~\textsc{i} &   2.420  &  -2.584   &    5.1 & HARPS \\
   4178.86                  & Fe~\textsc{ii}&   2.583  &  -2.510   &   39.3 & HARPS \\
   4233.17                  & Fe~\textsc{ii}&   2.583  &  -1.970   &   67.5 & HARPS \\
   4491.41                  & Fe~\textsc{ii}&   2.860  &  -2.710   &   22.7 & HARPS \\
   4515.34                  & Fe~\textsc{ii}&   2.844  &  -2.600   &   32.2 & HARPS \\
   4555.89                  & Fe~\textsc{ii}&   2.828  &  -2.400   &   39.1 & HARPS \\
   4576.34                  & Fe~\textsc{ii}&   2.840  &  -2.950   &   16.1 & HARPS \\
   4583.84\tablenotemark{a} & Fe~\textsc{ii}&   2.807  &   -1.93   &   65.5 & HARPS \\
   4620.52\tablenotemark{a} & Fe~\textsc{ii}&   2.830  &   -3.21   &    6.9 & HARPS \\
   5197.58                  & Fe~\textsc{ii}&   3.230  &  -2.220   &   29.8 & HARPS \\
   5234.63                  & Fe~\textsc{ii}&   3.220  &  -2.180   &   32.9 & HARPS \\
   5276.00                  & Fe~\textsc{ii}&   3.200  &  -2.010   &   40.6 & HARPS \\
   5325.55                  & Fe~\textsc{ii}&   3.220  &  -3.160   &    4.9 & HIRES \\
   5414.07                  & Fe~\textsc{ii}&   3.220  &  -3.580   &    2.1 & HIRES \\
   3437.28                  & Ni~\textsc{i} &   0.000  &  -1.207   &   79.6 & UVES  \\
   3472.54\tablenotemark{a} & Ni~\textsc{i} &   0.110  &  -0.790   &   89.0 & UVES  \\
   3483.77                  & Ni~\textsc{i} &   0.280  &  -1.120   &   73.2 & UVES  \\
   3500.85                  & Ni~\textsc{i} &   0.170  &  -1.294   &   72.1 & UVES  \\
   3519.77\tablenotemark{a} & Ni~\textsc{i} &   0.280  &  -1.422   &   68.8 & UVES  \\
   3597.71                  & Ni~\textsc{i} &   0.210  &  -1.115   &   77.1 & UVES  \\
   3807.14                  & Ni~\textsc{i} &   0.423  &  -1.220   &   74.5 & HARPS \\
   4605.00                  & Ni~\textsc{i} &   3.480  &  -0.290   &    7.6 & HARPS \\
   4686.22                  & Ni~\textsc{i} &   3.600  &  -0.640   &    2.2 & HARPS \\
   4904.41                  & Ni~\textsc{i} &   3.540  &  -0.170   &   10.6 & HARPS \\
   5081.11                  & Ni~\textsc{i} &   3.850  &   0.300   &   12.4 & HARPS \\
   5084.08                  & Ni~\textsc{i} &   3.680  &   0.030   &   10.2 & HARPS \\
   5115.40                  & Ni~\textsc{i} &   3.830  &  -0.110   &    6.6 & HARPS \\
   5155.76                  & Ni~\textsc{i} &   3.900  &  -0.090   &    4.8 & HARPS \\
   5476.90\tablenotemark{a} & Ni~\textsc{i} &   1.830  &  -0.890   &   48.5 & HARPS \\
   6643.64                  & Ni~\textsc{i} &   1.680  &  -2.300   &    4.8 & HARPS \\
   6767.77                  & Ni~\textsc{i} &   1.830  &  -2.170   &    4.8 & HARPS \\
   4680.14                  & Zn~\textsc{i} &   4.006  &  -0.830   &    3.4 & HARPS \\
   4722.16                  & Zn~\textsc{i} &   4.030  &  -0.370   &    8.4 & HARPS \\
   4810.54                  & Zn~\textsc{i} &   4.080  &  -0.160   &   14.5 & HARPS \\
\enddata
\tablenotetext{a}{EW measured but line rejected from abundance 
computation; see Section~\ref{analysis}.}
\tablecomments{Table~\ref{ewtab} is available in its entirety via the link
to the machine-readable table above.
 }              
\end{deluxetable}


==> tab14.tex <==
\begin{deluxetable*}{ccccccc}
\tablecaption{Wavelengths, excitation potentials, $\log(gf)$ values, 
and derived abundances
\label{linetab}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
%\rotate
\tablehead{
\colhead{Species} &
\colhead{Wavelength (\AA)\tablenotemark{a}} &
\colhead{E.P. (eV)} &
\colhead{$\log(gf)$} &
\colhead{$\log \epsilon$} &
\colhead{Instrument} &
\colhead{Ref.} }
\startdata
Be~\textsc{ii} &    3130.42  & 0.00     & -0.18          & -0.35 &  UVES   &  1  \\ 
Be~\textsc{ii} &    3131.07  & 0.00     & -0.48          & -0.38 &  UVES   &  1  \\ 
C~(CH)         & 4290--4325  & \nodata  & \nodata        & 6.51  &  HARPS  &  2  \\ 
N~(NH)         & 3357--3365  & \nodata  & \nodata        & 6.61  &  UVES   &  3  \\ 
O~(OH)         & 3110--3130  & \nodata  & \nodata        & 7.22  &  UVES   &  3  \\ 
Na~\textsc{i}  &    5682.63  & 2.10     & -0.71          & 4.56  &  HARPS  &  1  \\ 
Na~\textsc{i}  &    5688.20  & 2.10     & -0.41          & 4.61  &  HARPS  &  1  \\ 
Mg~\textsc{i}  &    4167.27  & 4.35     & -0.74          & 6.14  &  HARPS  &  4  \\ 
Mg~\textsc{i}  &    4702.99  & 4.33     & -0.44          & 5.57  &  HARPS  &  4  \\ 
Mg~\textsc{i}  &    5528.40  & 4.34     & -0.50          & 5.88  &  HARPS  &  4  \\ 
Mg~\textsc{i}  &    5711.09  & 4.34     & -1.72          & 5.91  &  HARPS  &  4  \\ 
Si~\textsc{i}  &    5701.10  & 4.93     & -2.05          & 5.94  &  HARPS  &  1  \\ 
Si~\textsc{i}  &    5708.40  & 4.93     & -1.47          & 5.92  &  HARPS  &  1  \\ 
Si~\textsc{i}  &    5772.15  & 5.06     & -1.75          & 5.86  &  HARPS  &  1  \\ 
Ca~\textsc{i}  &    4283.01  & 1.89     & -0.22          & 4.86  &  HARPS  &  1  \\ 
Ca~\textsc{i}  &    4318.65  & 1.89     & -0.21          & 4.74  &  HARPS  &  1  \\ 
Ca~\textsc{i}  &    4425.44  & 1.88     & -0.36          & 4.73  &  HARPS  &  1  \\ 
Ca~\textsc{i}  &    4434.96  & 1.89     & -0.01          & 4.67  &  HARPS  &  1  \\ 
Ca~\textsc{i}  &    4435.69  & 1.89     & -0.52          & 4.80  &  HIRES  &  1  \\ 
Ca~\textsc{i}  &    4454.78  & 1.90     & 0.26           & 4.63  &  HARPS  &  1  \\ 
Ca~\textsc{i}  &    4455.89  & 1.90     & -0.53          & 4.80  &  HARPS  &  1  \\ 
Ca~\textsc{i}  &    5588.76  & 2.52     & 0.21           & 4.91  &  HARPS  &  1  \\ 
Ca~\textsc{i}  &    5857.45  & 2.93     & 0.23           & 4.79  &  HARPS  &  1  \\ 
Ca~\textsc{i}  &    6102.72  & 1.88     & -0.85          & 4.79  &  HARPS  &  5  \\ 
Ca~\textsc{i}  &    6122.22  & 1.89     & -0.38          & 4.89  &  HARPS  &  5  \\ 
Ca~\textsc{i}  &    6162.17  & 1.90     & -0.17          & 4.91  &  HARPS  &  5  \\ 
Ca~\textsc{i}  &    6439.07  & 2.52     & 0.47           & 4.67  &  HARPS  &  1  \\ 
Sc~\textsc{ii} &    3576.34  & 0.01     & 0.01           & 1.62  &  UVES   &  6  \\ 
Sc~\textsc{ii} &    3590.47  & 0.02     & -0.55          & 1.74  &  UVES   &  6  \\ 
Sc~\textsc{ii} &    4246.84  & 0.32     & 0.24           & 1.36  &  HARPS  &  6  \\ 
Sc~\textsc{ii} &    4400.40  & 0.60     & -0.54          & 1.38  &  HARPS  &  6  \\ 
Sc~\textsc{ii} &    4415.56  & 0.59     & -0.67          & 1.41  &  HARPS  &  6  \\ 
Sc~\textsc{ii} &    4670.42  & 1.36     & -0.58          & 1.32  &  HARPS  &  6  \\ 
Sc~\textsc{ii} &    5526.79  & 1.77     & 0.02           & 1.34  &  HARPS  &  6  \\ 
Sc~\textsc{ii} &    5657.90  & 1.51     & -0.60          & 1.41  &  HARPS  &  6  \\ 
Ti~\textsc{i}  &    3998.64  & 0.05     & 0.01           & 3.31  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    4512.73  & 0.84     & -0.42          & 3.34  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    4518.02  & 0.83     & -0.27          & 3.28  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    4533.25  & 0.85     & 0.53           & 3.32  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    4534.78  & 0.84     & 0.34           & 3.28  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    4548.76  & 0.83     & -0.30          & 3.28  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    4555.49  & 0.85     & -0.43          & 3.24  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    4656.47  & 0.00     & -1.29          & 3.36  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    4681.91  & 0.05     & -1.02          & 3.24  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    4840.87  & 0.90     & -0.45          & 3.39  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    4981.73  & 0.84     & 0.56           & 3.30  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    4999.50  & 0.83     & 0.31           & 3.32  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    5016.16  & 0.85     & -0.52          & 3.29  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    5173.74  & 0.00     & -1.06          & 3.33  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    5192.97  & 0.02     & -0.95          & 3.33  &  HARPS  &  7  \\ 
Ti~\textsc{i}  &    5210.39  & 0.05     & -0.83          & 3.31  &  HARPS  &  7  \\ 
Ti~\textsc{ii} &    3321.70  & 1.23     & -0.31          & 3.38  &  UVES   &  8  \\ 
Ti~\textsc{ii} &    3343.76  & 0.15     & -1.15          & 3.54  &  UVES   &  8  \\ 
Ti~\textsc{ii} &    3491.05  & 0.11     & -1.15          & 3.61  &  UVES   &  8  \\ 
Ti~\textsc{ii} &    4028.34  & 1.89     & -0.96          & 3.49  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4394.06  & 1.22     & -1.78          & 3.46  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4395.03  & 1.08     & -0.54          & 3.49  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4395.84  & 1.24     & -1.93          & 3.40  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4399.77  & 1.24     & -1.19          & 3.51  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4417.71  & 1.17     & -1.19          & 3.52  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4418.33  & 1.24     & -1.97          & 3.47  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4443.80  & 1.08     & -0.72          & 3.62  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4444.55  & 1.12     & -2.24          & 3.47  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4450.48  & 1.08     & -1.52          & 3.51  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4464.45  & 1.16     & -1.81          & 3.48  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4470.85  & 1.17     & -2.02          & 3.35  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4533.96  & 1.24     & -0.53          & 3.55  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4571.97  & 1.57     & -0.32          & 3.56  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4583.41  & 1.16     & -2.92          & 3.43  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4636.32  & 1.16     & -3.02          & 3.37  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4657.20  & 1.24     & -2.24          & 3.42  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4708.66  & 1.24     & -2.34          & 3.51  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    4798.53  & 1.08     & -2.68          & 3.54  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    5129.16  & 1.89     & -1.24          & 3.34  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    5185.90  & 1.89     & -1.49          & 3.51  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    5226.54  & 1.57     & -1.26          & 3.47  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    5336.79  & 1.58     & -1.59          & 3.42  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    5381.02  & 1.57     & -1.92          & 3.42  &  HARPS  &  8  \\ 
Ti~\textsc{ii} &    5418.77  & 1.58     & -2.00          & 3.33  &  HARPS  &  8  \\ 
V~\textsc{i}   &    4379.23  & 0.30     & 0.55           & 2.08  &  HARPS  &  9  \\ 
V~\textsc{ii}  &    3951.96  & 1.48     & -0.78          & 2.30  &  HARPS  & 10  \\ 
V~\textsc{ii}  &    4005.71  & 1.82     & -0.52          & 2.39  &  HARPS  & 10  \\ 
Cr~\textsc{i}  &    3578.68  & 0.00     & 0.42           & 3.56  &  UVES   & 11  \\ 
Cr~\textsc{i}  &    4274.80  & 0.00     & -0.22          & 3.68  &  HARPS  & 11  \\ 
Cr~\textsc{i}  &    4289.72  & 0.00     & -0.37          & 3.53  &  HARPS  & 11  \\ 
Cr~\textsc{i}  &    4545.95  & 0.94     & -1.37          & 3.71  &  HARPS  & 11  \\ 
Cr~\textsc{i}  &    4646.15  & 1.03     & -0.74          & 3.67  &  HARPS  & 11  \\ 
Cr~\textsc{i}  &    4651.28  & 0.98     & -1.46          & 3.59  &  HARPS  & 11  \\ 
Cr~\textsc{i}  &    4789.34  & 2.54     & -0.33          & 3.68  &  HARPS  & 11  \\ 
Cr~\textsc{i}  &    5206.04  & 0.94     & 0.02           & 3.61  &  HARPS  & 11  \\ 
Cr~\textsc{i}  &    5296.69  & 0.98     & -1.36          & 3.61  &  HARPS  & 11  \\ 
Cr~\textsc{i}  &    5298.28  & 0.98     & -1.14          & 3.57  &  HARPS  & 11  \\ 
Cr~\textsc{i}  &    5345.80  & 1.00     & -0.95          & 3.62  &  HARPS  & 11  \\ 
Cr~\textsc{i}  &    5348.31  & 1.00     & -1.21          & 3.57  &  HARPS  & 11  \\ 
Cr~\textsc{i}  &    5409.77  & 1.03     & -0.67          & 3.62  &  HARPS  & 11  \\ 
Cr~\textsc{ii} &    4558.66  & 4.07     & -0.66          & 4.12  &  HARPS  & 12  \\ 
Cr~\textsc{ii} &    4588.21  & 4.07     & -0.83          & 4.03  &  HARPS  & 12  \\ 
Cr~\textsc{ii} &    4592.05  & 4.07     & -1.42          & 4.10  &  HARPS  & 12  \\ 
Mn~\textsc{i}  &    4041.35  & 2.11     & 0.28           & 3.19  &  HARPS  & 13  \\ 
Mn~\textsc{i}  &    4754.04  & 2.28     & -0.08          & 3.19  &  HARPS  & 13  \\ 
Mn~\textsc{i}  &    4762.37  & 2.89     & 0.30           & 3.17  &  HARPS  & 13  \\ 
Mn~\textsc{i}  &    4823.52  & 2.32     & 0.14           & 3.20  &  HARPS  & 13  \\ 
Mn~\textsc{i}  &    6021.82  & 3.08     & -0.05          & 3.18  &  HARPS  & 13  \\ 
Mn~\textsc{ii} &    3441.99  & 1.78     & -0.35          & 3.34  &  UVES   & 13  \\ 
Mn~\textsc{ii} &    3460.32  & 1.81     & -0.63          & 3.35  &  UVES   & 13  \\ 
Mn~\textsc{ii} &    3482.90  & 1.83     & -0.84          & 3.33  &  UVES   & 13  \\ 
Mn~\textsc{ii} &    3488.68  & 1.85     & -0.94          & 3.38  &  UVES   & 13  \\ 
Mn~\textsc{ii} &    3495.83  & 1.85     & -1.28          & 3.43  &  UVES   & 13  \\ 
Mn~\textsc{ii} &    3497.53  & 1.85     & -1.42          & 3.39  &  UVES   & 13  \\ 
Fe~\textsc{i}  &    3849.97  & 1.01     & -0.86          & 5.50  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    3865.52  & 1.01     & -0.95          & 5.56  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    3920.26  & 0.12     & -1.73          & 5.49  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    3922.91  & 0.05     & -1.63          & 5.47  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    3949.95  & 2.18     & -1.25          & 5.63  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4114.44  & 2.83     & -1.30          & 5.59  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4134.68  & 2.83     & -0.65          & 5.64  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4143.87  & 1.56     & -0.51          & 5.50  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4147.67  & 1.48     & -2.07          & 5.60  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4154.50  & 2.83     & -0.69          & 5.52  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4157.78  & 3.42     & -0.40          & 5.53  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4174.91  & 0.91     & -2.94          & 5.62  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4175.64  & 2.85     & -0.83          & 5.65  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4181.76  & 2.83     & -0.37          & 5.64  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4182.38  & 3.02     & -1.18          & 5.53  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4184.89  & 2.83     & -0.87          & 5.60  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4187.04  & 2.45     & -0.51          & 5.51  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4191.43  & 2.47     & -0.67          & 5.54  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4195.33  & 3.33     & -0.49          & 5.55  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4199.10  & 3.05     & 0.16           & 5.51  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4202.03  & 1.49     & -0.69          & 5.47  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4216.18  & 0.00     & -3.36          & 5.69  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4217.55  & 3.43     & -0.48          & 5.54  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4222.21  & 2.45     & -0.91          & 5.53  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4233.60  & 2.48     & -0.58          & 5.52  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4238.81  & 3.40     & -0.23          & 5.51  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4250.12  & 2.47     & -0.38          & 5.53  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4250.79  & 1.56     & -0.71          & 5.57  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4271.15  & 2.45     & -0.34          & 5.52  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4282.40  & 2.18     & -0.78          & 5.55  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4388.41  & 3.60     & -0.68          & 5.60  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4415.12  & 1.61     & -0.62          & 5.61  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4442.34  & 2.20     & -1.23          & 5.66  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4443.19  & 2.86     & -1.04          & 5.57  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4447.72  & 2.22     & -1.34          & 5.61  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4466.55  & 2.83     & -0.60          & 5.59  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4489.74  & 0.12     & -3.90          & 5.56  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4494.56  & 2.20     & -1.14          & 5.64  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4531.15  & 1.48     & -2.10          & 5.57  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4592.65  & 1.56     & -2.46          & 5.69  &  HIRES  & 14  \\ 
Fe~\textsc{i}  &    4595.36  & 3.29     & -1.76          & 5.58  &  HIRES  & 14  \\ 
Fe~\textsc{i}  &    4602.94  & 1.49     & -2.21          & 5.66  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4630.12  & 2.28     & -2.59          & 5.67  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4643.46  & 3.64     & -1.15          & 5.53  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4647.43  & 2.95     & -1.35          & 5.65  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4733.59  & 1.49     & -2.99          & 5.63  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4736.77  & 3.21     & -0.75          & 5.65  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4786.81  & 3.00     & -1.61          & 5.59  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4789.65  & 3.53     & -0.96          & 5.64  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4800.65  & 4.12     & -1.03          & 5.48  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4871.32  & 2.87     & -0.36          & 5.49  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4872.14  & 2.88     & -0.57          & 5.51  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4890.76  & 2.88     & -0.39          & 5.51  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4891.49  & 2.85     & -0.11          & 5.48  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4903.31  & 2.88     & -0.93          & 5.58  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4918.99  & 2.85     & -0.34          & 5.54  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4920.50  & 2.83     & 0.07           & 5.51  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4924.77  & 2.28     & -2.11          & 5.52  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4938.81  & 2.88     & -1.08          & 5.55  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4939.69  & 0.86     & -3.25          & 5.53  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4966.09  & 3.33     & -0.87          & 5.66  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    4994.13  & 0.92     & -2.97          & 5.58  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5006.12  & 2.83     & -0.62          & 5.52  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5028.13  & 3.56     & -1.12          & 5.53  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5044.21  & 2.85     & -2.02          & 5.49  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5049.82  & 2.28     & -1.36          & 5.58  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5051.63  & 0.92     & -2.76          & 5.63  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5068.77  & 2.94     & -1.04          & 5.58  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5079.22  & 2.20     & -2.11          & 5.69  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5083.34  & 0.96     & -2.84          & 5.55  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5123.72  & 1.01     & -3.06          & 5.64  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5127.36  & 0.92     & -3.25          & 5.61  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5131.47  & 2.22     & -2.52          & 5.58  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5141.74  & 2.42     & -2.24          & 5.63  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5150.84  & 0.99     & -3.04          & 5.55  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5151.91  & 1.01     & -3.32          & 5.66  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5166.28  & 0.00     & -4.12          & 5.62  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5171.60  & 1.49     & -1.72          & 5.61  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5191.45  & 3.04     & -0.55          & 5.51  &  HIRES  & 14  \\ 
Fe~\textsc{i}  &    5192.34  & 3.00     & -0.42          & 5.52  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5194.94  & 1.56     & -2.02          & 5.61  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5198.71  & 2.22     & -2.09          & 5.57  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5216.27  & 1.61     & -2.08          & 5.57  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5217.39  & 3.21     & -1.16          & 5.63  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5225.53  & 0.11     & -4.76          & 5.57  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5232.94  & 2.94     & -0.06          & 5.48  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5242.49  & 3.63     & -0.97          & 5.61  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5266.56  & 3.00     & -0.39          & 5.53  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5281.79  & 3.04     & -0.83          & 5.54  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5283.62  & 3.24     & -0.52          & 5.59  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5307.36  & 1.61     & -2.91          & 5.49  &  HIRES  & 14  \\ 
Fe~\textsc{i}  &    5339.93  & 3.27     & -0.72          & 5.61  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5364.87  & 4.45     & 0.23           & 5.60  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5367.47  & 4.42     & 0.44           & 5.49  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5379.57  & 3.69     & -1.51          & 5.52  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5410.91  & 4.47     & 0.40           & 5.48  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5497.52  & 1.01     & -2.83          & 5.65  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5501.47  & 0.96     & -3.05          & 5.66  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5506.78  & 0.99     & -2.79          & 5.68  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5586.76  & 3.37     & -0.14          & 5.55  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5662.52  & 4.18     & -0.57          & 5.65  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5701.54  & 2.56     & -2.14          & 5.55  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    5753.12  & 4.26     & -0.69          & 5.66  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6065.48  & 2.61     & -1.41          & 5.54  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6136.61  & 2.45     & -1.41          & 5.62  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6137.69  & 2.59     & -1.35          & 5.54  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6191.56  & 2.43     & -1.42          & 5.56  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6219.28  & 2.20     & -2.45          & 5.67  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6246.32  & 3.60     & -0.88          & 5.69  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6265.13  & 2.18     & -2.54          & 5.57  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6297.79  & 2.22     & -2.64          & 5.53  &  HIRES  & 14  \\ 
Fe~\textsc{i}  &    6393.60  & 2.43     & -1.58          & 5.63  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6421.35  & 2.28     & -2.01          & 5.60  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6430.85  & 2.18     & -1.95          & 5.56  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6494.98  & 2.40     & -1.24          & 5.64  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6592.91  & 2.73     & -1.47          & 5.53  &  HIRES  & 14  \\ 
Fe~\textsc{i}  &    6593.87  & 2.44     & -2.37          & 5.53  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6677.99  & 2.69     & -1.42          & 5.67  &  HARPS  & 14  \\ 
Fe~\textsc{i}  &    6750.15  & 2.42     & -2.58          & 5.65  &  HARPS  & 14  \\ 
Fe~\textsc{ii} &    4178.86  & 2.58     & -2.51          & 5.66  &  HARPS  & 15  \\ 
Fe~\textsc{ii} &    4233.17  & 2.58     & -1.97          & 5.80  &  HARPS  & 15  \\ 
Fe~\textsc{ii} &    4491.41  & 2.86     & -2.71          & 5.71  &  HARPS  & 15  \\ 
Fe~\textsc{ii} &    4515.34  & 2.84     & -2.60          & 5.81  &  HARPS  & 15  \\ 
Fe~\textsc{ii} &    4555.89  & 2.83     & -2.40          & 5.75  &  HARPS  & 15  \\ 
Fe~\textsc{ii} &    4576.34  & 2.84     & -2.95          & 5.73  &  HARPS  & 15  \\ 
Fe~\textsc{ii} &    5197.58  & 3.23     & -2.22          & 5.72  &  HARPS  & 15  \\ 
Fe~\textsc{ii} &    5234.63  & 3.22     & -2.18          & 5.73  &  HARPS  & 15  \\ 
Fe~\textsc{ii} &    5276.00  & 3.20     & -2.01          & 5.71  &  HARPS  & 15  \\ 
Fe~\textsc{ii} &    5325.55  & 3.22     & -3.16          & 5.68  &  HIRES  & 15  \\ 
Fe~\textsc{ii} &    5414.07  & 3.22     & -3.58          & 5.71  &  HIRES  & 15  \\ 
Co~\textsc{i}  &    3412.34  & 0.51     & 0.03           & 3.06  &  UVES   & 16  \\ 
Co~\textsc{i}  &    3412.63  & 0.00     & -0.78          & 3.31  &  UVES   & 16  \\ 
Co~\textsc{i}  &    3449.16  & 0.58     & -0.09          & 2.88  &  UVES   & 16  \\ 
Co~\textsc{i}  &    3529.03  & 0.17     & -0.90          & 3.00  &  UVES   & 17  \\ 
Co~\textsc{i}  &    3842.05  & 0.92     & -0.77          & 3.09  &  HARPS  & 16  \\ 
Co~\textsc{i}  &    3845.47  & 0.92     & 0.01           & 3.05  &  HARPS  & 16  \\ 
Co~\textsc{i}  &    4121.32  & 0.92     & -0.30          & 3.07  &  HARPS  & 17  \\ 
Ni~\textsc{i}  &    3437.28  & 0.00     & -1.21          & 4.33  &  UVES   & 18  \\ 
Ni~\textsc{i}  &    3483.77  & 0.28     & -1.12          & 4.27  &  UVES   &  1  \\ 
Ni~\textsc{i}  &    3500.85  & 0.17     & -1.29          & 4.30  &  UVES   & 18  \\ 
Ni~\textsc{i}  &    3597.71  & 0.21     & -1.12          & 4.27  &  UVES   & 18  \\ 
Ni~\textsc{i}  &    3807.14  & 0.42     & -1.22          & 4.30  &  HARPS  & 18  \\ 
Ni~\textsc{i}  &    4605.00  & 3.48     & -0.29          & 4.31  &  HARPS  &  1  \\ 
Ni~\textsc{i}  &    4686.22  & 3.60     & -0.64          & 4.20  &  HARPS  &  1  \\ 
Ni~\textsc{i}  &    4904.41  & 3.54     & -0.17          & 4.40  &  HARPS  &  1  \\ 
Ni~\textsc{i}  &    5081.11  & 3.85     & 0.30           & 4.29  &  HARPS  &  1  \\ 
Ni~\textsc{i}  &    5084.08  & 3.68     & 0.03           & 4.30  &  HARPS  &  1  \\ 
Ni~\textsc{i}  &    5115.40  & 3.83     & -0.11          & 4.37  &  HARPS  &  1  \\ 
Ni~\textsc{i}  &    5155.76  & 3.90     & -0.09          & 4.27  &  HARPS  &  1  \\ 
Ni~\textsc{i}  &    6643.64  & 1.68     & -2.30          & 4.30  &  HARPS  &  1  \\ 
Ni~\textsc{i}  &    6767.77  & 1.83     & -2.17          & 4.31  &  HARPS  &  1  \\ 
Cu~\textsc{i}  &    3247.53  & 0.00     & -0.06          & 1.39  &  UVES   & 19  \\ 
Cu~\textsc{i}  &    3273.95  & 0.00     & -0.36          & 1.40  &  UVES   & 19  \\ 
Cu~\textsc{ii} &    1979.96  & 2.83     & -0.59          & 2.00: &  STIS   & 20  \\ 
Cu~\textsc{ii} &    2037.13  & 2.83     & -0.23          & 1.74  &  STIS   & 20  \\ 
Cu~\textsc{ii} &    2054.98  & 2.93     & -0.29          & 1.77  &  STIS   & 20  \\ 
Cu~\textsc{ii} &    2104.80  & 2.97     & -0.51          & 1.93  &  STIS   & 20  \\ 
Cu~\textsc{ii} &    2112.10  & 3.25     & -0.11          & 1.95: &  STIS   & 20  \\ 
Cu~\textsc{ii} &    2126.04  & 2.83     & -0.23          & 1.85  &  STIS   & 20  \\ 
Zn~\textsc{i}  &    3075.90  & 0.00     & -3.85          & 2.81  &  UVES   &  1  \\ 
Zn~\textsc{i}  &    3302.58  & 4.03     & -0.02          & 2.75  &  UVES   & 21  \\ 
Zn~\textsc{i}  &    3345.01  & 4.08     & 0.26           & 2.70  &  UVES   & 21  \\ 
Zn~\textsc{i}  &    4680.14  & 4.01     & -0.85          & 2.76  &  HARPS  & 21  \\ 
Zn~\textsc{i}  &    4722.16  & 4.03     & -0.37          & 2.72  &  HARPS  & 21  \\ 
Zn~\textsc{i}  &    4810.53  & 4.08     & -0.15          & 2.82  &  HARPS  & 21  \\ 
Zn~\textsc{ii} &    2062.00  & 0.00     & -0.29          & 2.94  &  STIS   & 22  \\ 
Ge~\textsc{i}  &    1998.89  & 0.18     & -0.78          &$<$+1.5&  STIS   &  1  \\ 
Ge~\textsc{i}  &    2041.71  & 0.00     & -0.70          &$<$+1.4&  STIS   & 23  \\ 
Ge~\textsc{i}  &    2065.21  & 0.07     & -0.79          &$<$+1.2&  STIS   &  1  \\ 
As~\textsc{i}  &    1890.43  & 0.00     & -0.19          & 0.20  &  STIS   & 24  \\ 
As~\textsc{i}  &    1972.62  & 0.00     & -0.63          & 0.92  &  STIS   & 20  \\ 
As~\textsc{i}  &    1990.36  & 1.31     & -0.28          & 0.67  &  STIS   & 24  \\ 
Se~\textsc{i}  &    1960.89  & 0.00     & -0.43          & 1.47  &  STIS   & 23  \\ 
Se~\textsc{i}  &    2039.84  & 0.25     & -0.74          & 1.57  &  STIS   & 23  \\ 
Se~\textsc{i}  &    2074.78  & 0.00     & -2.26          & 1.63  &  STIS   & 23  \\ 
Sr~\textsc{i}  &    4607.33  & 0.00     & 0.28           & 0.85  &  HARPS  & 25  \\ 
Sr~\textsc{ii} &    4077.71  & 0.00     & 0.15           & 1.15  &  HARPS  &  1  \\ 
Sr~\textsc{ii} &    4161.79  & 2.94     & -0.47          & 1.32  &  HARPS  &  1  \\ 
Sr~\textsc{ii} &    4215.52  & 0.00     & -0.17          & 1.20  &  HARPS  &  1  \\ 
Y~\textsc{ii}  &    3549.01  & 0.13     & -0.29          & 0.33  &  UVES   & 26  \\ 
Y~\textsc{ii}  &    3584.52  & 0.10     & -0.42          & 0.33  &  UVES   & 26  \\ 
Y~\textsc{ii}  &    3600.74  & 0.18     & 0.34           & 0.28  &  UVES   & 26  \\ 
Y~\textsc{ii}  &    3601.91  & 0.10     & -0.15          & 0.27  &  UVES   & 26  \\ 
Y~\textsc{ii}  &    3611.04  & 0.13     & 0.05           & 0.23  &  UVES   & 26  \\ 
Y~\textsc{ii}  &    4398.01  & 0.13     & -0.75          & 0.08  &  HARPS  & 26  \\ 
Y~\textsc{ii}  &    4883.68  & 1.08     & 0.19           & 0.26  &  HARPS  & 26  \\ 
Y~\textsc{ii}  &    4900.11  & 1.03     & 0.03           & 0.25  &  HARPS  & 26  \\ 
Y~\textsc{ii}  &    5087.42  & 1.08     & -0.16          & 0.34  &  HARPS  & 26  \\ 
Y~\textsc{ii}  &    5200.41  & 0.99     & -0.47          & 0.14  &  HARPS  & 26  \\ 
Y~\textsc{ii}  &    5205.73  & 1.03     & -0.28          & 0.23  &  HARPS  & 26  \\ 
Zr~\textsc{ii} &    1996.74  & 0.71     & -0.04          & 1.00  &  STIS   & 27  \\ 
Zr~\textsc{ii} &    3095.07  & 0.04     & -0.84          & 1.00  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3129.76  & 0.04     & -0.54          & 1.07  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3273.05  & 0.16     & 0.30           & 1.00  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3279.26  & 0.10     & 0.12           & 0.95  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3284.71  & 0.00     & -0.37          & 1.08  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3404.83  & 0.36     & -0.49          & 1.04  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3430.53  & 0.47     & -0.16          & 1.07  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3457.56  & 0.56     & -0.47          & 1.06  &  UVES   & 27  \\ 
Zr~\textsc{ii} &    3479.39  & 0.71     & 0.18           & 1.04  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3481.15  & 0.80     & 0.29           & 0.94  &  UVES   & 27  \\ 
Zr~\textsc{ii} &    3496.20  & 0.04     & 0.26           & 0.99  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3505.67  & 0.16     & -0.39          & 1.06  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3551.95  & 0.10     & -0.36          & 1.08  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3556.59  & 0.47     & 0.07           & 0.98  &  UVES   & 28  \\ 
Zr~\textsc{ii} &    3998.96  & 0.56     & -0.52          & 1.09  &  HARPS  & 28  \\ 
Zr~\textsc{ii} &    4050.32  & 0.71     & -1.06          & 1.19  &  HARPS  & 28  \\ 
Zr~\textsc{ii} &    4149.20  & 0.80     & -0.04          & 1.11  &  HARPS  & 28  \\ 
Zr~\textsc{ii} &    4161.20  & 0.71     & -0.59          & 1.16  &  HARPS  & 28  \\ 
Zr~\textsc{ii} &    4208.98  & 0.71     & -0.51          & 1.12  &  HARPS  & 28  \\ 
Mo~\textsc{i}  &    3864.10  & 0.00     & -0.01          & 0.58  &  UVES   & 29  \\ 
Mo~\textsc{ii} &    2015.11  & 0.00     & -0.49          & 0.64  &  STIS   & 30  \\ 
Mo~\textsc{ii} &    2020.31  & 0.00     & 0.02           & 0.64  &  STIS   & 30  \\ 
Mo~\textsc{ii} &    2038.45  & 0.00     & -0.34          & 0.47  &  STIS   & 30  \\ 
Mo~\textsc{ii} &    2045.97  & 0.00     & -0.35          & 0.68  &  STIS   & 30  \\ 
Ru~\textsc{i}  &    3498.94  & 0.00     & 0.31           & 0.59  &  UVES   & 31  \\ 
Pd~\textsc{i}  &    3404.58  & 0.81     & 0.33           & -0.07 &  UVES   & 32  \\ 
Ag~\textsc{i}  &    3382.90  & 0.00     & -0.35          & -0.89: & UVES   & 33  \\ 
Cd~\textsc{ii} &    2144.39  & 0.00     & 0.02           & -0.03 &  STIS   & 20  \\ 
Te~\textsc{i}  &    2142.82  & 0.00     & -0.32          & 0.67: &  STIS   & 34  \\ 
Ba~\textsc{ii} &    4130.65  & 2.72     & 0.52           & 0.45  &  HARPS  & 35  \\ 
Ba~\textsc{ii} &    5853.69  & 0.60     & -0.91          & 0.42  &  HARPS  & 35  \\ 
La~\textsc{ii} &    3988.51  & 0.40     & 0.21           & -0.47 &  HARPS  & 36  \\ 
La~\textsc{ii} &    3995.74  & 0.17     & -0.06          & -0.31 &  HARPS  & 36  \\ 
La~\textsc{ii} &    4086.71  & 0.00     & -0.07          & -0.34 &  HARPS  & 36  \\ 
La~\textsc{ii} &    4123.22  & 0.32     & 0.13           & -0.33 &  HARPS  & 36  \\ 
Ce~\textsc{ii} &    3999.24  & 0.29     & 0.06           & -0.02 &  HARPS  & 37  \\ 
Ce~\textsc{ii} &    4073.47  & 0.48     & 0.21           & 0.11  &  HARPS  & 37  \\ 
Ce~\textsc{ii} &    4083.22  & 0.70     & 0.27           & 0.17  &  HARPS  & 37  \\ 
Ce~\textsc{ii} &    4137.65  & 0.52     & 0.40           & 0.02  &  HARPS  & 37  \\ 
Ce~\textsc{ii} &    4222.60  & 0.12     & -0.15          & 0.01  &  HARPS  & 37  \\ 
Ce~\textsc{ii} &    4486.91  & 0.29     & -0.18          & 0.19  &  HARPS  & 37  \\ 
Ce~\textsc{ii} &    4562.36  & 0.48     & 0.21           & 0.00  &  HARPS  & 37  \\ 
Ce~\textsc{ii} &    4572.28  & 0.68     & 0.22           & 0.13  &  HARPS  & 37  \\ 
Ce~\textsc{ii} &    4628.16  & 0.52     & 0.14           & -0.04 &  HARPS  & 37  \\ 
Nd~\textsc{ii} &    3784.24  & 0.38     & 0.15           & -0.12 &  UVES   & 38  \\ 
Nd~\textsc{ii} &    3826.41  & 0.06     & -0.41          & 0.08  &  UVES   & 38  \\ 
Nd~\textsc{ii} &    4109.45  & 0.32     & 0.35           & 0.01  &  HARPS  & 38  \\ 
Nd~\textsc{ii} &    4446.38  & 0.20     & -0.35          & -0.10 &  HARPS  & 38  \\ 
Sm~\textsc{ii} &    3568.27  & 0.48     & 0.29           & -0.42 &  UVES   & 39  \\ 
Sm~\textsc{ii} &    4434.32  & 0.38     & -0.07          & -0.61 &  HARPS  & 39  \\ 
Sm~\textsc{ii} &    4467.34  & 0.66     & 0.15           & -0.32 &  HARPS  & 39  \\ 
Eu~\textsc{ii} &    3724.93  & 0.00     & -0.09          & -0.85 &  UVES   & 40  \\ 
Eu~\textsc{ii} &    3819.67  & 0.00     & 0.51           & -0.83 &  HARPS  & 40  \\ 
Eu~\textsc{ii} &    3907.11  & 0.21     & 0.17           & -0.81 &  HARPS  & 40  \\ 
Eu~\textsc{ii} &    4129.72  & 0.00     & 0.22           & -0.76 &  HARPS  & 40  \\ 
Gd~\textsc{ii} &    3549.36  & 0.24     & 0.29           & -0.37 &  UVES   & 41  \\ 
Gd~\textsc{ii} &    3768.40  & 0.08     & 0.21           & -0.27 &  UVES   & 41  \\ 
Gd~\textsc{ii} &    4251.73  & 0.38     & -0.22          & -0.25 &  HARPS  & 41  \\ 
Dy~\textsc{ii} &    3531.71  & 0.00     & 0.77           & -0.21 &  UVES   & 42  \\ 
Dy~\textsc{ii} &    3536.02  & 0.54     & 0.53           & -0.17 &  UVES   & 42  \\ 
Dy~\textsc{ii} &    3550.22  & 0.59     & 0.27           & -0.16 &  UVES   & 42  \\ 
Dy~\textsc{ii} &    3563.15  & 0.10     & -0.36          & -0.20 &  UVES   & 42  \\ 
Dy~\textsc{ii} &    3694.81  & 0.10     & -0.11          & -0.27 &  UVES   & 42  \\ 
Dy~\textsc{ii} &    3944.68  & 0.00     & 0.11           & -0.17 &  HARPS  & 42  \\ 
Er~\textsc{ii} &    3830.48  & 0.00     & -0.22          & -0.41 &  HARPS  & 43  \\ 
Er~\textsc{ii} &    3896.23  & 0.06     & -0.12          & -0.31 &  HARPS  & 43  \\ 
Er~\textsc{ii} &    3906.31  & 0.00     & 0.12           & -0.34 &  HARPS  & 43  \\ 
Yb~\textsc{ii} &    2116.68  & 0.00     & -1.34          & -0.12: & STIS   & 44  \\ 
Yb~\textsc{ii} &    2126.74  & 0.00     & -0.87          & -0.42 &  STIS   & 45  \\ 
Yb~\textsc{ii} &    3694.20  & 0.00     & -0.30          & -0.49 &  UVES   & 46  \\ 
Os~\textsc{ii} &    2067.23  & 0.45     & -0.05          & -0.12: & STIS   & 47  \\ 
Ir~\textsc{ii} &    2126.81  & 0.00     & 0.07           & 0.35  &  STIS   & 47  \\ 
Pt~\textsc{i}  &    2049.39  & 0.00     & 0.02           & 0.35  &  STIS   & 20  \\ 
Pt~\textsc{i}  &    2067.51  & 0.00     & -0.62          & 0.54  &  STIS   & 48  \\ 
Pt~\textsc{i}  &    2103.34  & 0.10     & -0.15          & 0.37  &  STIS   & 48  \\ 
Hg~\textsc{ii} &    1927.27  & 0.00     & -0.40          &$<$+0.4&  STIS   & 20  \\ 
Pb~\textsc{i}  &    4057.81  & 1.32     & -0.22          &$<$+0.9&  HARPS  & 49  \\ 
\enddata                                       
\tablenotetext{a}{Air wavelengths are given for $\lambda >$~2000\,\AA\
and vacuum values below}                       
\tablerefs{
(1) \citealt{fuhr09};
(2) B.\ Plez, 2007, private communication;
(3) \citealt{kurucz95};
(4) \citealt{chang90};
(5) \citealt{aldenius09};
(6) \citealt{lawler89}, using hfs from \citealt{kurucz95};
(7) \citealt{blackwell82a,blackwell82b}, increased by 0.056~dex according to \citealt{grevesse89};
(8) \citealt{pickering01}, with corrections given in \citealt{pickering02};
(9) \citealt{doerr85}, using hfs from \citealt{kurucz95};
(10) \citealt{biemont89};
(11) \citealt{sobeck07};
(12) \citealt{nilsson06};
(13) \citealt{denhartog11} for both log($gf$) value and hfs;
(14) \citealt{obrian91};
(15) \citealt{melendez09};
(16) \citealt{cardon82}, using hfs from \citealt{kurucz95};
(17) \citealt{nitz99}, using hfs from \citealt{kurucz95};
(18) \citealt{blackwell89};
(19) \citealt{bielski75}, using hfs/IS from J.S.\ Sobeck et al.\ in prep.;
(20) this study;
(21) \citealt{kerkhoff80};
(22) \citealt{bergeson93};
(23) \citealt{morton00};
(24) \citealt{holmgren75}, using hfs from this study;
(25) \citealt{parkinson76};
(26) \citealt{biemont11};
(27) \citealt{malcheva06};
(28) \citealt{ljung06};
(29) \citealt{whaling88};
(30) \citealt{sikstrom01};
(31) \citealt{wickliffe94};
(32) \citealt{xu06};
(33) \citealt{fuhr09}, using hfs/IS from \citealt{hansen12};
(34) \citealt{roederer12a};
(35) \citealt{fuhr09}, using hfs/IS from \citealt{mcwilliam98} when available;
(36) \citealt{lawler01a}, using hfs from \citealt{ivans06} when available;
(37) \citealt{lawler09};
(38) \citealt{denhartog03}, using hfs/IS from \citealt{roederer08} when available;
(39) \citealt{lawler06}, using hfs/IS from \citealt{roederer08} when available;
(40) \citealt{lawler01b}, using hfs/IS from \citealt{ivans06};
(41) \citealt{denhartog06};
(42) \citealt{wickliffe00};
(43) \citealt{lawler08};
(44) $\log(gf)$ value from the Database on Rare Earths At Mons University (DREAM), using hfs/IS from this study;
(45) \citealt{kedzierski10}, using hfs/IS from this study;
(46) \citealt{sneden09} for both $\log(gf)$ and hfs/IS;
(47) \citealt{ivarsson04};
(48) \citealt{denhartog05};
% (49) \citealt{morton00}, using hfs/IS from this study;
(49) \citealt{biemont00}, using hfs/IS from \citealt{roederer12b}
}
%\tablecomments{Table~\ref{linetab} is available in its entirety via the link
%to the machine-readable table above.}                                            
\end{deluxetable*}


==> tab4.tex <==
Title: Detection of Elements at All Three r-process Peaks in the Metal-Poor Star
 HD 160617
Authors: Roederer I. U. and Lawler J.E., 
Table: Hyperfine structure line component patterns for 75As I.
================================================================================
Byte-by-byte Description of file: 
--------------------------------------------------------------------------------
   Bytes Format Units Label   Explanations
--------------------------------------------------------------------------------
  1-  9  F9.3   cm-1  WaveNum Center-of-Gravity Wavenumber
  11- 19 F9.4   0.1nm WaveVac Center-of-Gravity Vacuum Wavelength in Angstroms
  21     I1     ---   Fupp    Component upper level F or total angular momentum
  23     I1     ---   Flow    Component lower level F or total angular momentum
  25- 32 F8.5   cm-1  CWaveR  Component offset Wavenumber with respect to
                               Center-of-gravity Wavenumber
  34- 42 F9.6   0.1nm CWaveR  Component offset Wavelength with respect to
                               Center-of-gravity Wavelength
  44- 50 F7.5   ---   Str     Component strength (1)
--------------------------------------------------------------------------------
Note (1): Normalized to sum to one.
--------------------------------------------------------------------------------
50242.288 1990.3552 3 3  0.01800 -0.000713 0.35000
50242.288 1990.3552 3 2  0.06600 -0.002615 0.08750
50242.288 1990.3552 2 3 -0.05400  0.002139 0.08750
50242.288 1990.3552 2 2 -0.00600  0.000238 0.12500
50242.288 1990.3552 2 1  0.02600 -0.001030 0.10000
50242.288 1990.3552 1 2 -0.05400  0.002139 0.10000
50242.288 1990.3552 1 1 -0.02200  0.000872 0.02500
50242.288 1990.3552 1 0 -0.00600  0.000238 0.06250
50242.288 1990.3552 0 1 -0.04600  0.001822 0.06250
50693.897 1972.6240 2 3  0.02020 -0.000786 0.43750
50693.897 1972.6240 2 2  0.01356 -0.000527 0.15625
50693.897 1972.6240 2 1  0.00916 -0.000356 0.03125
50693.897 1972.6240 1 2 -0.02704  0.001052 0.15625
50693.897 1972.6240 1 1 -0.03144  0.001224 0.15625
50693.897 1972.6240 1 0 -0.03363  0.001309 0.06250
51610.393 1937.5942 3 3  0.02770 -0.001040 0.35000
51610.393 1937.5942 3 2  0.02106 -0.000790 0.08750
51610.393 1937.5942 2 3 -0.00260  0.000098 0.08750
51610.393 1937.5942 2 2 -0.00924  0.000347 0.12500
51610.393 1937.5942 2 1 -0.01364  0.000512 0.10000
51610.393 1937.5942 1 2 -0.02944  0.001105 0.10000
51610.393 1937.5942 1 1 -0.03384  0.001271 0.02500
51610.393 1937.5942 1 0 -0.03603  0.001353 0.06250
51610.393 1937.5942 0 1 -0.04394  0.001650 0.06250
52898.056 1890.4286 4 3  0.09685 -0.003461 0.37500
52898.056 1890.4286 3 3 -0.00115  0.000041 0.05833
52898.056 1890.4286 3 2 -0.00779  0.000279 0.23333
52898.056 1890.4286 2 3 -0.07465  0.002668 0.00417
52898.056 1890.4286 2 2 -0.08129  0.002905 0.07292
52898.056 1890.4286 2 1 -0.08569  0.003062 0.13125
52898.056 1890.4286 1 2 -0.13029  0.004656 0.00625
52898.056 1890.4286 1 1 -0.13469  0.004814 0.05625
52898.056 1890.4286 1 0 -0.13688  0.004892 0.06250


==> tab8.tex <==
Title: Detection of Elements at All Three r-process Peaks in the Metal-Poor Star
 HD 160617
Authors: Roederer I.U. and Lawler J.E.,
Table: Hyperfine structure and isotopic line component patterns for Cd II lines
================================================================================
Byte-by-byte Description of file:
--------------------------------------------------------------------------------
   Bytes Format Units Label   Explanations
--------------------------------------------------------------------------------
  1- 9   F9.3   cm-1  WaveNum Center-of-Gravity Wavenumber
  11- 19 F9.4   0.1nm WaveAir Center-of-Gravity Air Wavelength in Angstroms
  21- 23 F3.1   ---   Fupp    Component upper level F or total angular momentum
  25- 27 F3.1   ---   Flow    Component lower level F or total angular momentum
  29- 36 F8.5   cm-1  CWaveR  Component offset Wavenumber with respect to
                               Center-of-gravity Wavenumber
  38- 46 F9.6   0.1nm CWaveR  Component offset Wavelength with respect to
                               Center-of-gravity Wavelength
  48- 54 F7.5   ---   Str     Component strength (1)
  56- 58 I3     ---   Iso     Isotope
--------------------------------------------------------------------------------
Note (1): Normalized to sum to one.
--------------------------------------------------------------------------------
44136.173 2265.0145 0.5 0.5  0.07759 -0.003982 0.01250 106
44136.173 2265.0145 0.5 0.5  0.05164 -0.002650 0.00890 108
44136.173 2265.0145 0.5 0.5  0.02684 -0.001378 0.12490 110
44136.173 2265.0145 0.5 0.5  0.00224 -0.000115 0.24130 112
44136.173 2265.0145 0.5 0.5 -0.01955  0.001003 0.28730 114
44136.173 2265.0145 0.5 0.5 -0.03603  0.001849 0.07490 116
44136.173 2265.0145 1.0 1.0  0.12588 -0.006461 0.06400 111
44136.173 2265.0145 1.0 0.0 -0.35880  0.018415 0.03200 111
44136.173 2265.0145 0.0 1.0  0.20349 -0.010444 0.03200 111
44136.173 2265.0145 1.0 1.0  0.10568 -0.005424 0.06110 113
44136.173 2265.0145 1.0 0.0 -0.40133  0.020598 0.03055 113
44136.173 2265.0145 0.0 1.0  0.18687 -0.009591 0.03055 113
46618.532 2144.3943 1.5 0.5  0.07759 -0.003570 0.01250 106
46618.532 2144.3943 1.5 0.5  0.05164 -0.002376 0.00890 108
46618.532 2144.3943 1.5 0.5  0.02684 -0.001235 0.12490 110
46618.532 2144.3943 1.5 0.5  0.00224 -0.000103 0.24130 112
46618.532 2144.3943 1.5 0.5 -0.01955  0.000899 0.28730 114
46618.532 2144.3943 1.5 0.5 -0.03603  0.001657 0.07490 116
46618.532 2144.3943 2.0 1.0  0.13557 -0.006237 0.08000 111
46618.532 2144.3943 1.0 1.0  0.16146 -0.007428 0.01600 111
46618.532 2144.3943 1.0 0.0 -0.32321  0.014869 0.03200 111
46618.532 2144.3943 2.0 1.0  0.11582 -0.005328 0.07638 113
46618.532 2144.3943 1.0 1.0  0.14290 -0.006574 0.01527 113
46618.532 2144.3943 1.0 0.0 -0.36411  0.016751 0.03055 113

